ManiFPT: Defining and Analyzing Fingerprints of Generative Models

Recent works have shown that generative models leave traces of their underlying generative process on the generated samples, broadly referred to as fingerprints of a generative model, and have studied their utility in detecting synthetic images from real ones. However, the extend to which these fingerprints can distinguish between various types of synthetic image and help identify the underlying generative process remain under-explored. In particular, the very definition of a fingerprint remains unclear, to our knowledge. To that end, in this work, we formalize the definition of artifact and fingerprint in generative models, propose an algorithm for computing them in practice, and finally study its effectiveness in distinguishing a large array of different generative models. We find that using our proposed definition can significantly improve the performance on the task of identifying the underlying generative process from samples (model attribution) compared to existing methods. Additionally, we study the structure of the fingerprints, and observe that it is very predictive of the effect of different design choices on the generative process.

==> rqs/rq1b-visualize-artifacts.tex <==
% \subsection{Visualization of artifacts and fingerprints of generative models under our definition} \label{sec:rq1b}
We visualize the artifacts and fingerprints of generative models under our definition.
Fig.~\ref{fig:viz-our-art-rgb-gm64} and Fig.~\ref{fig:viz-our-art-rgb-gm256} show examplary pairs of ($x_g$, $x_p$ (projection), artifact) for each generative model in our datasets, GM64 and GM256, respectively. \todo{see more in appendix for gn-ffhq; maybe keep just gm256 on main, if space limited; or show art in rgb, and art in freq (currently in appendix) both of gm256}




==> tbls/tbl-our-gm-set.tex <==

\begin{table}[h!]
  \centering
  \caption{List of models in our dataset of GM (trained on CelebA)}
\label{tbl:our-GM-set}
% \begin{tabular}{|p{0.1\textwidth}|p{0.8\textwidth}|}
% \begin{tabular}{ll}
\begin{tabular}{p{0.1\textwidth}p{0.8\textwidth}}
    \toprule
    Class      & Models \\ 
    \midrule
    VAE        & $\beta$-VAE\cite{Higgins2017betaVAELB}, DFC-VAE\cite{Hou2017DeepFC}, FactorVAE\cite{Kim2018DisentanglingBF}, InfoVAE\cite{Zhao2017InfoVAEIM}, NVAE\cite{Vahdat2020NVAEAD}                \\
    \midrule
    GAN        & plain GAN (pGAN)\cite{Goodfellow2014GenerativeAN}, EBGAN\cite{Zhao2016EnergybasedGA}, DCGAN \cite{Radford2016UnsupervisedRL}, LSGAN\cite{Mao2017LeastSG}, WGAN-gp/lp\cite{Gulrajani2017ImprovedTO}, DRAGAN-gp/lp\cite{kodali2017convergence}, StyleGAN\cite{Karras2019ASG}, StyleGAN2\cite{Karras2020AnalyzingAI}, ProGAN\cite{Karras2018ProgressiveGO}, MMDGAN\cite{Binkowski2018DemystifyingMG}, SNGAN\cite{Miyato2018SpectralNF}, InfoMaxGAN\cite{Lee2021InfoMaxGANIA} \\ 
    \midrule
    Flow       & GLOW\cite{Kingma2018GlowGF}, MaCow\cite{Ma2019MaCowMC}  \\ 
    \midrule
    Score & Noise Conditional Score Network (NCSN) \cite{Song2019GenerativeMB}, Guided Diffusion \cite{Dhariwal2021DiffusionMB}   \\ 
    \bottomrule
\end{tabular}
\end{table}
